Fairness by design in shared-energy allocation problems

This paper studies how to aggregate prosumers (or large consumers) and their collective decisions in electricity markets, with a focus on fairness. Fairness is essential for prosumers to participate in aggregation schemes. Some prosumers may not be able to access the energy market directly, even though it would be beneficial for them. Therefore, new companies offer to aggregate them and promise to treat them fairly. This leads to a fair resource allocation problem. We propose to use acceptability constraints to guarantee that each prosumer gains from the aggregation. Moreover, we aim to distribute the costs and benefits fairly, taking into account the multi-period and uncertain nature of the problem. Rather than using financial mechanisms to adjust for fairness issues, we focus on various objectives and constraints, within decision problems, that achieve fairness by design. We start from a simple single-period and deterministic model, and then generalize it to a dynamic and stochastic setting using, e.g., stochastic dominance constraints.

==> cover.tex <==
% \documentclass[a4paper,12pt, oneside]{article}

% \usepackage[utf8]{inputenc}
% \usepackage[english]{babel}
% \usepackage{amsmath,amsfonts,amssymb, amsthm,bbm}

% \title{Cover Letter for\\
% ``Policy with guaranteed risk-adjusted performance for multistage stochastic linear problems''\\
% submitted to \textsc{Computational Management Science}}

% \author{Zoé Fornier (METRON, France),
%  Vincent Lecl\`{e}re (École des Ponts, France),
%  Pierre Pinson (Imperial College)}

% \begin{document}
% To the editors of the special edition ``Optimization under Uncertainty'' of Computational Management Science,

% We are submitting this paper for publication in the special edition ``Optimization under Uncertainty'' of Computational Management Science, because its subject is very closely related to the presentation given by Zoé Fornier at the 2023 International Conference on Stochastic Programming.

% The paper discuss various way of modelling fairness considerations in optimization model. 
% The motivating example is the aggregation of electric prosumers, but it can be easily adapted to other settings. 
% We claim that fairness by design can be incorporated in the model through two tools: acceptability constraints that ensures that each agent is getting something out of the aggregation; and aggregation operators that fairly distribute gains made by the aggregation.
% One of the highlight of the paper is to discuss reasonable extension of these constraints to a dynamic or a stochastic setting, leveraging stochastic dominance theory.

% \bigskip

% Thank you very much for your consideration,

% Zoé Fornier,
%  Vincent Lecl\`{e}re,
%  and Pierre Pinson 
% \end{document}

% vim:set spelllang=en:


==> figure_results_deterministic.tex <==
\begin{tikzpicture}

    \begin{scope}[local bounding box = minimax robust]

    \foreach \y in {-1, 0, ..., 5}
    \draw[very thin, color=black!50, dashed] (-0.2, \y) -- (10.5, \y);

    \foreach \x in {2, 4, ..., 10}
    \draw[very thin, color=black!50, dashed] (\x, -1.5) -- (\x, 5.5);

    \foreach \y in {-1, 1,2, 3, 4, 5}
    \node[] at (-0.6, \y) {$\y0 \%$};
    \node[] at (-0.4, 0) {$0 \%$};

    \draw[ very thick] (0,0) -- (11,0);
    \draw (10,0) node[below]{};
    \draw[->, very thick] (0,-1.2) -- (0,6.5);
    \node[text centered, text width = 2.5cm] at (-1.3,6.3) {Savings (\%)};

    \node[red] at (2, 0) {\large \textbf{\ding{110}}};
    \node[red] at (4, 0) {\large \textbf{\ding{110}}};
    \node[red] at (6, 0) {\large \textbf{\ding{110}}};
    \node[red] at (8, 0) {\large \textbf{\ding{110}}};
    \node[red] at (10, 0) {\large \textbf{\ding{110}}};

    \node[orange] at (2, 0) {\large \textbf{\ding{115}}};
    \node[orange] at (4,0) {\large \textbf{\ding{115}}};
    \node[orange] at (6,0) {\large \textbf{\ding{115}}};
    \node[orange] at (8, 0) {\large \textbf{\ding{115}}};
    \node[orange] at (10, 0) {\large \textbf{\ding{115}}};

    \node[blue] at (2, 0) {\large \textbf{\ding{108}}};
    \node[blue] at (4, 0) {\large \textbf{\ding{108}}};
    \node[blue] at (6, 0) {\large \textbf{\ding{108}}};
    \node[blue] at (8, 0) {\large \textbf{\ding{108}}};
    \node[blue] at (10, 0) {\large \textbf{\ding{108}}};
    
    % \invisible{
    %     \node[PurpleMetron] (c1) at (12, 4.6) {\Large \textbf{\ding{110}}};
    %     \node[OrangeMetron] (c2) at (12, 3.6) {\Large \textbf{\ding{115}}};
    %     \node[Flame] (c3) at (12, 2.6) {\Large \textbf{\ding{108}}};
    
    %     \node[PurpleMetron] [right = 0cm of c1] { \large $c_{A_1}$};
    %     \node[OrangeMetron] [right = 0cm of c2] { \large $c_{A_2}$};
    %     \node[Flame] [right = 0cm of c3] {\large $c_{A_1}+c_{A_2}$};
    % }

    \node[] at (5, 6.8) {\Large \textbf{Robust minimax}};

    \node[] at (2, -2) {\Large $\preceq_{\emptyset}$};
    \node[] at (4, -2) {\Large $\preceq_{\EE}$};
    \node[] at (6, -2) {\Large $\preceq_{ic}$};
    \node[] at (8, -2) {\Large $\preceq_{(1)}$};
    \node[] at (10, -2) {\Large $\preceq_{as}$};

    \end{scope}

\end{tikzpicture}

==> literature.tex <==
In this section, we give a general overview of how fairness is defined and modeled across the scientific literature, while making the link to our energy application. 
We first cover some definitions of fairness, before diving into the existing mathematical treatment of the subject.

First, we present two examples to illustrate the concepts introduced in this section.

\vspace{2mm}
\begin{example}[Multiportfolio management]
    An advisor is in charge of $N$ portfolios with individual interests across various assets.
    The aggregation of portfolios can be modeled with the following optimization model: 
    \begin{subequations}
        \begin{align}
        \Max_{\change{\na{x_i}_{i \in [N]}}} \quad & \sum_{i \in [N]} r_i(x_i) - c\Bp{\sum_{i \in [N]} x_i} \\
        & x_i \in \cX_i & \forall i \in [N],
    \end{align}
    \end{subequations}
where $x_i$ are the trades of $i$, constrained to be in set $\cX_i$, $r_i$ is the revenue function, and $c$ the trading cost function. 
    %\vl{j'ai ajouté un function de coût de trading explicite}
    \label{example:multiportfolio}
\end{example}

\vspace{2mm}
\begin{example}[Shared Energy storage system (ESS) management]
    A manager is in charge of managing an ESS, in which $M$ buildings have invested collaboratively.
    \new{This example is inspired by the problem presented in \cite{NJB}}.
    We model the aggregation of buildings with:
    \begin{subequations}
         \begin{align}
        \Min_{\change{\na{x_t^j}_{j \in [M], t \in [T]}}} \quad & \sum_{t\in [T]} \; \sum_{j \in [M]} \; c_t^j q_t^j \\
        & p_t^j + \phi_t^j + q_t^j \geq d_t^j & \forall t \in [T],\forall j \in [M] \\
        & x_t^j:=(p_t^j,\phi_t^j,q_t^j) \in \cX_t^j & \forall t \in [T] \forall j \in [M] \\
        & SoC_t = SoC_{t-1} + \sum_{j \in [M]} \phi_t^j & \forall t \in [T], \label{eq:SESS-soc}
    \end{align}
    \end{subequations}
    %\vl{You lack the storage dynamic}
    where a building $j$ is modeled by $d_t^j$, its energy demand at time $t$; $p_t^j$, its energy production at $t$; $q_t^j$, the  quantity of energy bought from the grid at price $c_t^j$; and \change{$\phi_t^j$, if positive (resp. negative), is the quantity of energy charged to (resp. discharged from) the ESS at $t$.}
    All variables at $t$ are constrained by set $\cX_t^j$.
    Finally, $SoC_t$ is the \change{State of Charge} in the shared battery at $t$, modeled with dynamic equations \eqref{eq:SESS-soc}.
    \label{example:ess}
\end{example}

\vspace{2mm}
In both those examples, to make all participants benefit from the aggregation, the aggregator must ensure fair treatment.
In \cref{example:multiportfolio}, the advisor must guarantee equitable distribution of market costs among portfolios. 
In \cref{example:ess}, deciding how energy from the shared battery should be allocated is not straightforward \new{as it affects directly the cost of each prosumer. 
Therefore, the aggregator’s choices regarding prosumer access to energy storage has to be fair:
}
should access be proportional to each building's investments, based on energy needs, or should alternative criteria be considered?

\subsection{Defining, modeling and accommodating fairness}

In the Oxford Dictionary, fairness is defined as \textit{the quality of treating people equally or in a way that is reasonable}.
The definition is simple but subjective.
Is treating people equally, regardless of any token of individuality, considered fair in society?
Furthermore, what does it mean to be reasonable? 
Whatever take we have on fairness is necessarily subjective and context-dependent.
We present here some notions of the philosophical approach to fairness (see \cite{Kon2003} for a deeper analysis). 
We do not pretend to give a thorough description of the philosophical literature, 
but merely outline some concepts relevant to the following work.

\temporary{Fair process}
When speaking of fairness, \cite{Kon2003} distinguish \emph{fair processes} from \emph{fair outcomes}.
\new{By opposition to fairness, we call \textit{unfair} a process or an outcome that is not fair.}
In the first paradigm, 
fairness is evaluated not through the outcomes, but through the treatment of each individual in the group that results in said outcomes.  
This concept is relevant in Machine Learning, for applications like granting or denying loans, bail or parole decisions etc.
In such problems, the inherent biases in the data used for algorithm training can lead to unfair predictive outcomes, 
\change{in the sense that individuals of a given social class are favored compared to others.} 
Hence, it becomes imperative to integrate fairness into the learning process and think of ways to assess fairness across different data populations.
We refer to \cite{JJK+2017,CH2020,RTK2023a} for more details on the way fairness can be addressed in machine learning. 

\temporary{Fair outcomes}
On the other hand, the \emph{fair outcomes} paradigm takes into consideration the individual outcomes and makes sure that everyone gets their fair share. 
This approach is favored in game theory where each individual (or player) is modeled with a utility function whose actual value depends on the actions of all players.
For a given set of actions, we obtain a utility vector, denoted $u:=(u_1, \dots, u_n)$, representing every agent's utility $u_i$. 
A utility vector is then said to be \emph{fair} if it satisfies a set of properties that might vary from one specific fairness definition to another.
\new{Among them, individual rationality is key as it ensures every individual is better off in the aggregation, and therefore accepts to be a part of it.}
In \cref{example:multiportfolio}, the utility is the benefit of each agent,
whereas in \cref{example:ess} the utility is the energy costs of each building. 
In the remainder of this paper, we discuss fair outcomes approaches.

\temporary{Egalitarism}
Intuitively, fairness can be confused with \textit{Egalitarianism} where 
a utility vector is said to be fair if all coordinates are equal, meaning that everyone gets the same share.
For instance, the \textit{Gini coefficient} \citep{Gini} 
is a commonly used indicator to measure equality---mistaken for fairness---  which evaluates how far a given distribution is from the equal distribution.
Although it makes sense in some applications,
it is impractical most of the time since people have unequal access to resources and different needs.
indeed, in \cref{example:ess}, if we consider equality through the quantity of energy given from the ESS, we would add constraints ensuring everyone gets the exact same amount of energy:
 \begin{align*}
    &  \sum_{t=1}^T \phi_t^j = \sum_{t=1}^T \phi_t^{j'} \, &  \forall j \neq j'.
\end{align*}
We can see the limits of such modeling as it would provide too much energy to buildings with smaller energy consumption. 
Moreover, it is found to be unpopular in surveys (\cite{Kon2003}), as people feel they get less than they should.
Thus, equal resource (and opportunity) distribution does not \change{always} address social inequality.

\temporary{The Need Principle}
To counteract these side effects, the \textit{Need Principle} aims at satisfying basic needs equally first and then focusing on efficiency. 
This is a trade-off between need and other distributive goals. 
In \cref{example:ess}, each building could decompose its energy demand $d_t^j$ into the minimum energy needed $n_t^j$ plus energy asked for comfort $s_t^j$.
Then, additional constraints \eqref{eq:SESS-need} can be added to the aggregation model to ensure that everyone gets free energy to satisfy its needs:
 \begin{align*}
    & p_t^j + \phi_t^j + q_t^j \geq n_t^j + s_t^j & \forall t \in [T],\forall j \in [M], \\
    & p_t^j + \phi_t^j \geq n_t^j & \forall t \in [T],\forall j \in [M]. \label{eq:SESS-need} \\
\end{align*}
Then, depending on the energy available in the ESS and the energy produced by each building, the manager dispatches the energy to minimize the aggregated costs of energy bought to the grid. The Need Principle finds practical application in Euphemia \cite{euphemia}, an algorithm developed to optimize the orders to be executed on the European coupled electricity market.
Euphemia pursues a dual objective: 
first, equitably distributing curtailment among areas where a portion of orders are unaccepted;
and second, maximizing social welfare by optimizing the total market value in the Day-Ahead auction.
The emphasis is on maximizing order acceptance for each area, 
and then the algorithm seeks an efficient solution.

\temporary{The Minimax approach}
A different approach %called the \emph{social contract}\vl{two names ?}, 
was introduced by \cite{Raw71}:
assuming that a group of individuals has no idea of their rank or situation in society,
they will agree on a social contract aiming at maximizing the well-being of the least well-off. 
If the agents possess distinct characteristics, 
it might be difficult to compare them and ensure equitable treatment among them.
This approach to fairness is often referred to as \textit{minimax fairness}, as this amounts to optimizing the worst objective among agents.
In \cref{example:multiportfolio}, the minimax aggregator is modeled as:
%\vl{how to deal with transaction costs? Currently there is no interaction between agents.}
\begin{subequations}
    \begin{align}
    \Max_{x,t} \qquad & \min_i \; \na{\,  r_i(x_i) - t_i\, }\\
    \text{s.t.}\qquad & x_i \in \cX_i & \forall i \in [N] \\
    & \sum_{i \in [N]} t_i = c \left(\sum_{i \in [N]} x_i \right), \label{eq:portofolios-tradingshared}
\end{align}
\end{subequations}
where $t_i$ represents what the aggregation charges portfolio $i$ for trading.
Then, \eqref{eq:portofolios-tradingshared} ensures the sum of cost charged to portfolios equals to the trading cost of the aggregation. 
This amounts to having transfer variables in-between agents, 
which is proposed by \cite{IT2014} to solve a multi-portfolio problem with fairness considerations.
We avoid transfer variables in this paper, as they may raise privacy and trust concerns in practical application. 
Instead, we simplify the approach by designating the aggregator as the sole entity with complete information on the problem.

Now that we have presented some of the philosophical concepts that define the foundations of fairness, we discuss in the following mathematical ways to model and assess fairness.

\subsection{Mathematical models of fairness}
\label{subsec:literature_historic}

\subsubsection{Notions of fair solutions}
\temporary{Pareto optimality for multi-objective problems, for instance, balance between fair and efficient}
For more than a century, fairness or inequality has been widely discussed in the literature.
The first fairness notion can be traced back to:
%\citet{Pareto}
a utility vector is said to be Pareto optimal if there are no other accessible utility vector where an individual is better off without negatively impact another. 
Pareto optimality does not imply fairness in a solution, but guarantees a stability. 
This concept is also used when trying to find a balance between multiple objectives: 
traditionally in portfolio management to find a trade-off between a high expected revenue and low risk.
In our context, 
this can be adapted as we look for a trade-off between the total revenue of the aggregation (efficiency) and the fairness of the solution.
%see \citet{LWA2022} and \citet{KFWM2021}.


\temporary{game theory: Nash solution}
One of the main challenges facing fairness is resource allocation among agents.
This naturally falls into the scope of game theory. 
In a founding article \citep{Nash}, John Nash introduced the bargaining problem
where two \new{rational} agents, allowed to bargain, try to maximize the sum of their utilities. 
\new{Agents are rationals, hence individual rationality is ensured through a \textit{disagreement point}, which is the strategy decided by players if they cannot reach an agreement.}
As agents can cooperate, they must have an agreement on properties a utility vector, $u$, should satisfy.
Nash proposed four axioms to constitute this agreement:
\textit{Pareto optimality};
\textit{Symmetry}, applying the same permutation to two utility vectors does not change their order;
\textit{Independence of irrelevant alternatives}, if a utility vector is the optimal utility vector within the feasible set, it remains so if the set is reduced.
\textit{Scale invariance}: applying affine transformations to the utility vector does not change the social ranking. 
Then, he showed that, under a number of assumptions (among them, the set of feasible utility vectors must be convex and compact),
there exists a unique utility vector satisfying those axioms. 
This unique utility vector is regarded in the literature as a viable option when seeking fairness.
It has been demonstrated that under convexity of the feasible set, it can be obtained by maximizing the product of utilities (\cite{Nas1953,Mut1999}), and thus by maximizing a logarithmic sum of utilities:
\begin{align*}
    \max_{u \in \cU} & \quad \sum_{i=1}^N \log(u_i - d_i), 
\end{align*}
where $u\in \cU$ is a feasible utility vectors among $N$ players, and $d$ the disagreement point.
This approach is referred to as \textit{proportional fairness}.
Some papers criticized the \textit{Independence of irrelevant alternatives} for having undesirable side effects. 
To overcome those issues, \cite{Kalai} proposed to replace it with a \textit{monotonicity} axiom, resulting in another unique utility vector,
and a slightly different vision on fairness.

\temporary{game theory: Cooperative games and shapley values}
In opposition to bargaining games, cooperative games study games where forming coalitions is allowed. 
In this theory, it is assumed that players can achieve superior outcomes by cooperating \delete{rather than working against each other.}
Players must establish their common interest and then work together to achieve it, 
which requires information exchanges.
In \cite{P-295}, Shapley studied a class of functions that evaluate players participation in a coalition. 
Considering a set of axioms (symmetry, efficiency and law of aggregation), Shapley showed that there exists a unique value function satisfying those axioms.
He derived an explicit formula to compute the value of a player $i$ in a cooperative game with a set $N$ of players: 
\begin{align*}
    \phi_i(v) = \sum_{S \subset N \setminus \na{i}} \binom{|N|-1}{|S|}^{-1} \, \bp{v(S \cup \na{i}) - v(S)},
\end{align*}
where $v(S)$ gives the total expected sum of payoffs the cooperation $S$ can obtain.
The values obtained $\na{\phi_i(v)}_{i \in N}$ are called Shapley values.
They are considered as a fair redistribution of gains in the group. 
However, they are very hard to compute in practice (as the size of the problem grows, those values are not computable).

\subsubsection{Evaluating the fairness of outcomes}

\temporary{game theory: measure of fairness ($\alpha-$fairness, ...)} 
As we study fairness, we naturally look for ways to measure it. 
In \cite{lan2009axiomatic}, the authors proposed a mathematical framework based on five axioms (continuity, homogeneity, saturation, partition and starvation) to define and evaluate fairness measures of utility vectors. 
They established a class of functions satisfying those axioms, which comprises various known measures on fairness, such as 
Atkinson's index, $\alpha-$fairness, Jain's index etc.
Removing the axiom of homogeneity, this class is extended to measures looking for a trade-off between fairness and efficiency.
Although a variety of indices exist, the Gini coefficient, mentioned before, is the most commonly used. 
For example, in a recent paper \citep{HOP+2019} studying the fairness in power system reliability,  
the authors compared a Gini-based index to a variance-based index (similar to the standard deviation index).

\temporary{The price of fairness}
When fairness is considered in the problem (through the objective or constraints), it comes at a price: a fair solution might not be the most efficient one. 
Indeed, many articles try to find a balance between efficiency (have the best objective possible) and fairness (have a fair solution). 
In \cite{BFT2011}, the authors established bounds on the price of fairness for two approaches (proportional fairness and minimax fairness) in resource allocation problems among self-interested players.


\temporary{Reference for a more complete overview}
In this section, we referred to work that lay the foundations of fairness modeling in mathematics. 
For a more complete review, we refer to \cite{Hoo} where the authors provided guidelines for readers to choose the appropriate definition and modeling of fairness.
They went through the list of indicators and criteria that exist to measure and define fairness.
However, they assumed that fairness can always be reflected through the social welfare function (which corresponds to utilities in game theory) of agents. 
This means that the well-being of different agents are comparable through a single value.

In the following section, we present some applications of aggregations and the way fairness is considered or evaluated. 

\subsection{Applications of fairness in the literature}
%\zfil{je ne suis pas satisfaite de la section, j'ai l'impression que les paragraphes ne vont pas bien ensemble}

% \zfil{Manque \cite{CBGK2015} (-> dans secion 2.2 avec Nash bargaining solution), where the authors study the fairness of energy allocation among electric vehicles in a charging stations network.
% The challenge is to determine a charging protocol which prioritizes access to electrical power to a fleet of vehicles, while managing congestion, and taking account of fairness in the allocation among users.
% They compare a utilitarian approach to the problem (maximizing the flow protocol) to a (weighted) proportional fairness one. }

\temporary{For simplicity, the utilitarian approach is usually chosen.}
In this article, we focus on an approach \textit{by-design}, meaning that fairness is already accommodated in an optimization model. 
Although fairness is commonly recognized as crucial, in most articles the approach adopted derives from act utilitarianism: 
one should at every moment promote the greatest aggregate happiness, which consists in maximizing social welfare regardless of individual costs.
For instance, in \cite{XIAO2020115159}, the authors studied an aggregator in charge of multiple agents within a power system.
They optimized the total revenue of the aggregation without considering the impact on each agent individually. 
In \cite{MP2019}, an aggregator of prosumers can focus on different indicators (import/export costs, exchange with the system operator, peak-shaving services etc.) to optimize its trades with the energy market, and the trades between prosumers.
The indicator to focus on must be agreed on by the prosumers.
The authors gave a sensitivity analysis on the parameters of the problem to determine what would increase the social acceptability of such an aggregation system. 
However, the model is utilitarian as it does not consider the distribution of costs among agents.

%\zfil{This paragraph is the one I am not sure about: maybe more sense to be with paragraph on cooperation games, and talk about nucleolus and core}
\temporary{Coalitional games.}
Other articles have proposed to first optimize the problem and then \change{handle fairness through benefit post-allocation schemes.}
\new{One way to deal with post-allocation is to }
model the aggregation as a coalitional game.
This is the case of \cite{FSLB2015}, where the authors studied a risk-averse renewable-energy multi-portfolio problem. 
In order to get a fair and stable allocation of profits, they chose \textit{the Nucleolus} approach which finds a vector utility that minimizes the incentive to leave the aggregation for the worst coalition.
In particular, this solution is in \textit{the core} of the game, meaning every players gains from staying in the grand coalition.
Similarly, in \cite{YHS2021}, the authors studied a group of buildings with solar generation that mutually invest in an ESS. 
The approach is to, first, optimize the problem formulated as a two-stage stochastic coalition game.
Then, a fair reallocation of costs is determined by computing the nucleolus distribution which minimizes the minimal dissatisfaction of agents.

\temporary{Post allocation schemes}
Some papers \change{propose different methods to elaborate} post-allocation schemes.
For example in \cite{YFLM2023}, the authors studied the joint participation of wind farms with a shared energy storage. 
The solution is found by first solving a two-stage stochastic program, 
and then reallocating the lease cost among users in a proportional scheme.
They chose to make a wind farm pay depending on its increase of revenue after using the energy storage leasing service.
In \cite{WZW+2019a}, the authors valued cooperation in their model, which is another way to look at cost redistribution.  
They considered an aggregator which participates in capacity and energy market for a number of energy users.
In their model, the aggregator is not in charge of the users decisions but of the trades with the energy market, 
therefore he must incentivize users to deviate from their optimal scheduling for minimizing total revenue. 
They proposed to solve an asymmetric Nash bargaining problem to determine the incentizing costs.

\temporary{Fairness in the constraints}
Typically, fairness is dealt with through the objective function, or in a post-allocation scheme. 
However, some researchers proposed constraints to ensure fairness.
For example in \cite{AKY2022}, the authors constrained the allocation feasibility set for a resource allocation problem. 
They introduced a welfare function dominance constraint: 
the admissible set of social welfare functions must dominate a referenced one.
Then, with a utilitarian objective, a trade-off  between fairness and efficiency is obtained.
An alternative approach, proposed in \cite{Oh2022}, is to bound a fairness indicator. 
The authors studied the energy planning of multiple agents over a virtual energy storage system (VESS), where energy dispatch is managed by an aggregator. 
They introduced two fairness indicators depending on the energy allocation, and added constraints bounding them in a utilitarian model. 
Then, they compared the results with a minimax approach, where they optimize the minimal fairness indicator over agents. 

\temporary{Stochastic considerations}
%\cite{WZW+2019a,FSLB2015}
In many cases, uncertainties are inherent to the problem. 
If multiple articles have dealt with uncertainties, they rarely have a stochastic take on fairness. 
For example, in both \cite{YFLM2023} and \cite{YHS2021}, the authors solved their problem with a two-stage program and then redistributed the costs fairly after uncertainty realization. 
Thus, there is no stochastic policy for fair redistribution. 
Other articles accommodated risk-averse profiles to game theory approaches. 
In \cite{GKW2023}, the authors studied a risk-averse extension of the Bargaining Problem. 
They adapted Nash bargaining axioms to constrain the feasible utility vectors depending on the risk profile of players.
%\zfil{Manque \cite{WZW+2019a,FSLB2015}}



==> nomenclature.tex <==
Deterministic
\begin{itemize}
    \item $\setProsumer$ is the set of prosumer indexed by $\indexProsumer$
    \item $\decisionProsumer{\indexProsumer}$ is the set of state and decision variables modeling prosumer $\indexProsumer$
    \item $\constraintProsumer{\indexProsumer}$ is modeling the constraints of prosumer $\indexProsumer$
    \item $\objectiveProsumer{\indexProsumer}$ is the objective of prosumer $\indexProsumer$
    \item $\constraintMarket$ is modeling market constraints
    \item $\modelProsumer{\indexProsumer}$ is the model for prosumer $\indexProsumer$ alone, of optimal value $\valueProsumer{\indexProsumer}$
    \item $\objectiveUtilitarian$ is the utilitarian function
    \item $\objectiveMinimax$ is the minimax function
    \item $\objectiveProportional$ is the proportional function
    \item $\coefficientAcceptability$ is the coefficient of acceptability for the acceptability constraints
    \item $\modelAggregator$ is the model for the aggregator
\end{itemize}

Dynamic
\begin{itemize}
    \item $\horizon$ is the number of stages in the problem, time is indexed by $\indexTime$
    \item $\modelAggregatorDynamic{\indexTime}$ is the dynamic model for the aggregator
    \item $\modelProsumerDynamic{\indexTime}{\indexProsumer}$ is the dynamic for the prosumer $\indexProsumer$ of optimal value $\valueProsumerDynamic{\indexTime}{\indexProsumer}$
    \item $\instantaneousCostProsumer{\indexTime}{\indexProsumer}$ is the function modeling costs at stage $\indexTime$
    \item $\actualizationRate$ is an actualization rate coefficient of instantaneous costs in the objective
    \item $\decisionProsumerDynamic{\indexTime}{\indexProsumer}$ is the decisions variables in the dynamic setting for prosumer $\indexProsumer$ at stage $\indexTime$, composed of state variables $\stateProsumerDynamic{\indexTime}{\indexProsumer}$ and control variables $\controlProsumer{\indexTime}{\indexProsumer}$
    \item $\constraintProsumerDynamic{\indexTime}{\indexProsumer}$ models the constraints of prosumer $\indexProsumer$ at stage $\indexTime$
    \item $\dynamicFunctionProsumer{\indexTime}{\indexProsumer}$ models the dynamic constraints linking state variables
    \item $\constraintMarketDynamic{\indexTime}$ models the constraints on the energy market at stage $\indexTime$
\end{itemize}

On small illustration:
\begin{itemize}
    \item $\quantityEnergyDAExample{\indexStage}{\indexProsumer}$ is the quantity of energy bought at price $\pricesDAExample{\indexStage}$ on the day-ahead market for prosumer $\indexProsumer$ at $\indexStage$
    \item $\quantityEnergyBExample{\indexStage}{\indexProsumer}$ is the quantity of energy bought at price $\pricesBExample{\indexStage}$ on the balancing market for prosumer $\indexProsumer$ at $\indexStage$
    \item $\buyDA{\indexStage}$ is the binary variable equal to $1$ if prosumer $i$ buys energy on the day-ahead market at time $\indexStage$, and $0$ otherwise.
\end{itemize}




==> old_files/main_old.tex <==
% \documentclass{article}
% %\documentclass[sn-mathphys,Numbered]{sn-jnl}
% \usepackage{graphicx} % Required for inserting images
% \usepackage[utf8]{inputenc}
% %\usepackage[left=3cm,right=3cm,]{geometry}
% \usepackage{booktabs}

% \usepackage{float}
% %Pour les titres de figures
% \usepackage{caption}
% \captionsetup[figure]{font=normalsize}
% %Pour les Figures
% \usepackage{tikz}
% \usetikzlibrary{arrows,petri,topaths,shapes,snakes,decorations,fit,positioning,patterns}

% \usepackage{amsmath} %Pour certaines formules de maths
% \usepackage{amsthm} %Pour les théorèmes
% \usepackage{amssymb} %Pour symboles comme esperance
% \usepackage{bm} %Pour mettre en gras qqc dans une équation
% \usepackage{lscape} %Pour avoir des pages horizontales
% \usepackage[linesnumbered, onelanguage, ruled, vlined]{algorithm2e}
% %Pour les titres de figures
% \usepackage{caption}
% \captionsetup[figure]{font=normalsize}
% \usepackage[toc,page]{appendix} 
% \usepackage{todonotes}
% \usepackage{hyperref}
% \usepackage{cleveref}
% \usepackage{subcaption}
% \usepackage[authordate]{biblatex-chicago}
% \usepackage{pifont}
% \usepackage{pgfplots}

% %\addbibresource{bibliography.bib}
% \bibliography{bibliography}

% \input{command.sty}

% \title{Fairness-Aware Shared-Energy Allocation Under Uncertainty: A Stochastic Programming Approach}
% \author{Zoé Fornier, Vincent Leclère, Pierre Pinson}

% \date{}

% \begin{document}

% \maketitle

% %\section*{Abstract}
% \input{abstract}

% \tableofcontents

% \section{Introduction}
% \input{introduction}

% % \zfil{
% % Skeleton of this section
% % \begin{itemize}
% %     \item An introduction going over the definition of fairness in a broad sense. As no one agrees on a single definition, and as the perception of fairness changes depending on the context, it a complicated notion that needs to be studied carefully.
% %     Give different take on fairness.
% %     \item A section on historical concepts on the theory of fairness in mathematical modeling: Gini index, Pareto optimality, Nash's bargaining solution, Shapley's values, The price of fairness. 
% %     \begin{itemize}
% %         \item One section on criterias evaluating fairness
% %         \item Another on ways to model it
% %     \end{itemize}
% %     \item Game Theory: fairness easily modeled in games. Axioms ensuring in a sense fairness, cooperative games, non self-interested players...
% %     \item Fairness in optimization problems: social welfare functions representing a view on fairness; trade-off between efficiency and fairness; modeling through constraints. 
% %     \item Applications: fairness in multi-portfolio management, VSS management, group investments, machine learning \dots
% % \end{itemize}
% % }


% \section{What is fairness?}
% \label{sec:fairness}
% \input{literature}

% \section{A shared-resource allocation problem in the context of a prosumer aggregator}
% \label{sec:problem}
% \input{deterministic}

% \section{Time-consistent fairness in a dynamic setting}
% \label{sec:dynamic}
% \input{dynamic}

% \section{Accommodating fairness to uncertainties with stochastic optimization}
% \label{sec:stochastic}
% \input{stochastic}

% \section{Conclusion}
% \label{sec:conclusion}
% \input{conclusion}


% \section*{Nomenclature}
% \input{nomenclature}

% \printbibliography


% \end{document}


==> old_files/old_example.tex <==
\subsection{Illustration}
\label{subsec:deterministic_illustration}

We now illustrate in a small example the implications of each model proposed in this section.
We consider a problem with two consumers ($\setProsumer := \na{1,2}$) and $\nbStages:=5$ stages.
Consumer $1$ has a fixed energy load of $5$MWh while Consumer $2$ has a final demand of $10$MWh but is flexible: 
at each time, he can consume up to $5$MWh.
Together they can access the day-ahead market, which requires a minimum of $7$MWh. 

At each stage $\indexStage$, we must decide how much energy $\quantityEnergyDAExample{\indexStage}{\indexProsumer}$ (\textit{resp.} $\quantityEnergyBExample{\indexStage}{\indexProsumer}$) to purchase from the day-ahead (\textit{resp.} balancing) market for consumer $\indexProsumer$.
To model the minimum volume requirement for the day-ahead market, we introduce binary variables $buyDA{\indexStage}$ representing the decision to buy a day-ahead. 
The objective for consumer $\indexProsumer$ is to minimize its energy costs:
\begin{subequations}
\begin{align}
    \objectiveProsumer{\indexProsumer}(\decisionProsumer{\indexProsumer}) = \sum_{\indexStage=1}^\nbStages \nc{\, \pricesDAExample{\indexStage} \quantityEnergyDAExample{\indexStage}{\indexProsumer} + \pricesBExample{\indexStage} \quantityEnergyBExample{\indexStage}{\indexProsumer} \,} ,
\end{align}
where $\pricesDAExample{\indexStage}$ (\textit{resp.} $\pricesBExample{\indexStage}$) is the price of energy at $\indexStage$ on the day-ahead (\textit{resp.} balancing) market.
We obtain the very simple aggregated model: 

    \begin{align}
        \Min_{\decisionProsumer{ }} \quad & \objectiveProsumer{ }(\decisionProsumer{ })  \\
        \text{s.c} \quad & \quantityEnergyDAExample{\indexStage}{1} + \quantityEnergyBExample{\indexStage}{A_1} = 5 & \forall \indexStage \in [5], \\
        & 0 \leq \quantityEnergyDAExample{\indexStage}{2} + \quantityEnergyBExample{\indexStage}{2} \leq 5 & \forall \indexStage  \in [5], \\
        & \sum_{\indexStage=1}^5 (\quantityEnergyDAExample{\indexStage}{2} + \quantityEnergyBExample{\indexStage}{2}) = 5, \\
        & 7 \buyDA{\indexStage} \leq \quantityEnergyDAExample{\indexStage}{1} + \quantityEnergyDAExample{\indexStage}{2} \leq M \, \buyDA{\indexStage} & \forall \indexStage  \in [5], \\
        & \buyDA{\indexStage} \in \na{0,1} & \forall \indexStage  \in [5],
    \end{align}
\end{subequations}
where $\objectiveProsumer{ }$ is the chosen objective for the aggregation. 
We solve this small problem with the utilitarian function $\objectiveUtilitarian$, with the minimax function $\objectiveMinimax$ and with the proportional function $\objectiveProportional$.
Then, we add average, progressive and stage-wise acceptability constraints to the model with $\coefficientAcceptability=1$. 

\begin{figure}[H]
    \hspace{-2cm}
    \input{figures/toy_example.tex}
\end{figure}

\zfil{Mettre aussi acceptability constraints results, mais seulement utilitarian?}

Firstly, it's worth noting that none of the consumers can individually access the day-ahead market. 
In the utilitarian solution,the primary focus lies in minimizing aggregated costs,
making it optimal to always consistently access the day-ahead market as a group. 
To achieve this, consumer $2$ redistributes their energy load across the $5$ time steps, incurring a higher individual cost than when acting independently. 
Conversely, the proportional objective function adopts a more bargaining-oriented approach, resulting in collaboration only during time slots when consumer $2$ intends to consume. 
This leaves consumer $1$ to operate independently during other time slots, resulting in limited savings compared to the utilitarian approach.
Lastly, the minimax approach finds a middle ground, 
where consumer $2$ assists consumer $1$ on most time steps but withdraws support on some occasions, allowing them to avoid expensive consumption.
In this case, both consumers achieve similar proportional savings, amounting to approximately 35\% compared to operating independently.

